Formal Verification of Quantum Programs: Theory, Tools and Challenges

Over the past 27 years, quantum computing has seen a huge rise in interest from both academia and industry. At the current rate, quantum computers are growing in size rapidly backed up by the increase of research in the field. Significant efforts are being made to improve the reliability of quantum hardware and to develop suitable software to program quantum computers. In contrast, the verification of quantum programs has received relatively less attention. Verifying programs is especially important in the quantum setting due to how difficult it is to program complex algorithms correctly on resource-constrained and error-prone quantum hardware. Research into creating verification frameworks for quantum programs has seen recent development, with a variety of tools implemented using a collection of theoretical ideas. This survey aims to be a short introduction into the area of formal verification of quantum programs, bringing together theory and tools developed to date. Further, this survey examines some of the challenges that the field may face in the future, namely the development of complex quantum algorithms.

==> Images/tikz_zx_hh.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [] (0) at (-9, 12) {};
		\node [] (2) at (-9, 6) {};
		\node [] (4) at (-7, 12) {};
		\node [] (6) at (-7, 6) {};
		\node [style=gn] (28) at (-7, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (29) at (-7, 7.75) {$\frac{\pi}{2}$};
		\node [style=rn] (30) at (-7, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (31) at (-7, 8.5) {$\frac{\pi}{2}$};
		\node [style=rn] (32) at (-7, 11) {$\frac{\pi}{2}$};
		\node [style=rn] (33) at (-7, 9.5) {$\frac{\pi}{2}$};
		\node [] (34) at (-5, 12) {};
		\node [] (35) at (-5, 6) {};
		\node [style=gn] (36) at (-5, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (37) at (-5, 7.75) {$\frac{\pi}{2}$};
		\node [style=rn] (38) at (-5, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (39) at (-5, 9) {$\pi$};
		\node [style=rn] (40) at (-5, 11) {$\frac{\pi}{2}$};
		\node [] (41) at (-3, 12) {};
		\node [] (42) at (-3, 6) {};
		\node [style=gn] (43) at (-3, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (44) at (-3, 9) {$-\frac{\pi}{2}$};
		\node [style=rn] (45) at (-3, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (46) at (-3, 7.75) {$\pi$};
		\node [style=rn] (47) at (-3, 11) {$\frac{\pi}{2}$};
		\node [] (48) at (-9, 5) {};
		\node [] (49) at (-9, -1) {};
		\node [style=gn] (51) at (-9, 2) {};
		\node [style=rn] (52) at (-9, 0) {$-\frac{\pi}{2}$};
		\node [style=rn] (54) at (-9, 4) {$\frac{\pi}{2}$};
		\node [] (55) at (-7, 5) {};
		\node [] (56) at (-7, -1) {};
		\node [style=rn] (58) at (-7, 0) {$-\frac{\pi}{2}$};
		\node [style=rn] (59) at (-7, 4) {$\frac{\pi}{2}$};
		\node [] (60) at (-5, 5) {};
		\node [] (61) at (-5, -1) {};
		\node [style=rn] (62) at (-5, 2) {};
		\node [] (63) at (-3, 5) {};
		\node [] (64) at (-3, -1) {};
		\node [style=had] (66) at (-9, 8) {};
		\node [style=had] (68) at (-9, 10) {};
		\node [] (69) at (-8.5, 9) {};
		\node [] (70) at (-7.5, 9) {};
		\node [] (71) at (-7.5, 9) {};
		\node [] (72) at (-6.5, 9) {};
		\node [] (73) at (-5.5, 9) {};
		\node [] (74) at (-5.5, 9) {};
		\node [] (75) at (-4.5, 9) {};
		\node [] (76) at (-3.5, 9) {};
		\node [] (77) at (-3.5, 9) {};
		\node [] (78) at (-8.5, 2) {};
		\node [] (79) at (-7.5, 2) {};
		\node [] (80) at (-7.5, 2) {};
		\node [] (81) at (-6.5, 2) {};
		\node [] (82) at (-5.5, 2) {};
		\node [] (83) at (-5.5, 2) {};
		\node [] (84) at (-4.5, 2) {};
		\node [] (85) at (-3.5, 2) {};
		\node [] (86) at (-3.5, 2) {};
		\node [] (fl) at (-2.5, 9) {};
		\node [] (fldots) at (-1.5, 9) {$\dots$};
		\node [] (sl) at (-9.5, 2) {};
		\node [] (sldots) at (-10.5, 2) {$\dots$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (32);
		\draw (32) to (28);
		\draw (28) to (33);
		\draw (33) to (31);
		\draw (31) to (29);
		\draw (29) to (30);
		\draw (30) to (6.center);
		\draw (34.center) to (40);
		\draw (40) to (36);
		\draw (39) to (37);
		\draw (37) to (38);
		\draw (38) to (35.center);
		\draw (36) to (39);
		\draw (41.center) to (47);
		\draw (47) to (43);
		\draw (45) to (42.center);
		\draw (46) to (45);
		\draw (46) to (44);
		\draw (44) to (43);
		\draw (48.center) to (54);
		\draw (52) to (49.center);
		\draw (52) to (51);
		\draw (51) to (54);
		\draw (55.center) to (59);
		\draw (58) to (56.center);
		\draw (59) to (58);
		\draw (62) to (61.center);
		\draw (60.center) to (62);
		\draw (63.center) to (64.center);
		\draw (0.center) to (68);
		\draw (68) to (66);
		\draw (66) to (2.center);
		\draw [-stealth] (69.center) to (71.center);
		\draw [-stealth] (72.center) to (74.center);
		\draw [-stealth] (75.center) to (77.center);
		\draw [-stealth] (78.center) to (80.center);
		\draw [-stealth] (81.center) to (83.center);
		\draw [-stealth] (84.center) to (86.center);
		\draw (fl.center) to (fldots);
		\draw [-stealth] (sldots) to (sl.center);
	\end{pgfonlayer}
\end{tikzpicture}


==> Images/tikz_zx_inf.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [] (0) at (0.5, 5.25) {};
		\node [] (1) at (0.5, 6.25) {};
		\node [style=had] (2) at (0.5, 5.75) {};
		\node [] (3) at (2, 4.5) {};
		\node [] (4) at (2, 7) {};
		\node [style=rn] (5) at (2, 5) {$\frac{\pi}{2}$};
		\node [style=rn] (6) at (2, 6.5) {$\frac{\pi}{2}$};
		\node [style=gn] (7) at (2, 5.75) {$\frac{\pi}{2}$};
		\node [] (8) at (1.25, 5.75) {=};
		\node [] (9) at (-1.5, 3.5) {};
		\node [] (10) at (-1, 3.5) {...};
		\node [] (11) at (-0.5, 3.5) {};
		\node [] (12) at (-1.5, 4.5) {};
		\node [] (13) at (-1, 4.5) {...};
		\node [] (14) at (-0.5, 4.5) {};
		\node [style=rn] (15) at (-1, 4) {$\alpha$};
		\node [] (16) at (-0.25, 3.25) {};
		\node [] (17) at (0.25, 3.25) {...};
		\node [] (18) at (0.75, 3.25) {};
		\node [] (19) at (-0.25, 4.25) {};
		\node [] (20) at (0.25, 4.25) {...};
		\node [] (21) at (0.75, 4.25) {};
		\node [style=rn] (22) at (0.25, 3.75) {$\beta$};
		\node [] (23) at (1.75, 3.25) {};
		\node [] (24) at (2.25, 3.25) {...};
		\node [] (25) at (2.75, 3.25) {};
		\node [] (26) at (1.75, 4.25) {};
		\node [] (27) at (2.25, 4.25) {...};
		\node [] (28) at (2.75, 4.25) {};
		\node [style=rn] (29) at (2.25, 3.75) {$\alpha + \beta$};
		\node [] (30) at (1.25, 3.75) {=};
		\node [style=rn] (31) at (4.25, 3.75) {};
		\node [] (32) at (4.25, 3.25) {};
		\node [] (33) at (4.25, 4.25) {};
		\node [] (34) at (4.75, 3.75) {=};
		\node [] (35) at (5.25, 3.25) {};
		\node [] (36) at (5.25, 4.25) {};
		\node [style=gn] (37) at (4.25, 6) {$\alpha$};
		\node [] (38) at (4.25, 5) {};
		\node [] (39) at (4.25, 6.5) {};
		\node [] (40) at (4.75, 5.75) {=};
		\node [style=rn] (41) at (4.25, 5.5) {$\pi$};
		\node [style=gn] (42) at (5.25, 5.5) {$-\alpha$};
		\node [] (43) at (5.25, 6.5) {};
		\node [] (44) at (5.25, 5) {};
		\node [style=rn] (45) at (5.25, 6) {$\pi$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (0.center) to (2);
		\draw (2) to (1.center);
		\draw (3.center) to (5);
		\draw (5) to (7);
		\draw (7) to (6);
		\draw (6) to (4.center);
		\draw (9.center) to (15);
		\draw (11.center) to (15);
		\draw (15) to (14.center);
		\draw (15) to (12.center);
		\draw (16.center) to (22);
		\draw (18.center) to (22);
		\draw (22) to (21.center);
		\draw (22) to (19.center);
		\draw (15) to (22);
		\draw (23.center) to (29);
		\draw (25.center) to (29);
		\draw (29) to (28.center);
		\draw (29) to (26.center);
		\draw (32.center) to (31);
		\draw (31) to (33.center);
		\draw (36.center) to (35.center);
		\draw (37) to (39.center);
		\draw (38.center) to (41);
		\draw (41) to (37);
		\draw (42) to (44.center);
		\draw (43.center) to (45);
		\draw (45) to (42);
	\end{pgfonlayer}
\end{tikzpicture}


==> Images_eps/tikz_zx_hh.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [] (0) at (-9, 12) {};
		\node [] (2) at (-9, 6) {};
		\node [] (4) at (-7, 12) {};
		\node [] (6) at (-7, 6) {};
		\node [style=gn] (28) at (-7, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (29) at (-7, 7.75) {$\frac{\pi}{2}$};
		\node [style=rn] (30) at (-7, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (31) at (-7, 8.5) {$\frac{\pi}{2}$};
		\node [style=rn] (32) at (-7, 11) {$\frac{\pi}{2}$};
		\node [style=rn] (33) at (-7, 9.5) {$\frac{\pi}{2}$};
		\node [] (34) at (-5, 12) {};
		\node [] (35) at (-5, 6) {};
		\node [style=gn] (36) at (-5, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (37) at (-5, 7.75) {$\frac{\pi}{2}$};
		\node [style=rn] (38) at (-5, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (39) at (-5, 9) {$\pi$};
		\node [style=rn] (40) at (-5, 11) {$\frac{\pi}{2}$};
		\node [] (41) at (-3, 12) {};
		\node [] (42) at (-3, 6) {};
		\node [style=gn] (43) at (-3, 10.25) {$\frac{\pi}{2}$};
		\node [style=gn] (44) at (-3, 9) {$-\frac{\pi}{2}$};
		\node [style=rn] (45) at (-3, 7) {$\frac{\pi}{2}$};
		\node [style=rn] (46) at (-3, 7.75) {$\pi$};
		\node [style=rn] (47) at (-3, 11) {$\frac{\pi}{2}$};
		\node [] (48) at (-9, 5) {};
		\node [] (49) at (-9, -1) {};
		\node [style=gn] (51) at (-9, 2) {};
		\node [style=rn] (52) at (-9, 0) {$-\frac{\pi}{2}$};
		\node [style=rn] (54) at (-9, 4) {$\frac{\pi}{2}$};
		\node [] (55) at (-7, 5) {};
		\node [] (56) at (-7, -1) {};
		\node [style=rn] (58) at (-7, 0) {$-\frac{\pi}{2}$};
		\node [style=rn] (59) at (-7, 4) {$\frac{\pi}{2}$};
		\node [] (60) at (-5, 5) {};
		\node [] (61) at (-5, -1) {};
		\node [style=rn] (62) at (-5, 2) {};
		\node [] (63) at (-3, 5) {};
		\node [] (64) at (-3, -1) {};
		\node [style=had] (66) at (-9, 8) {};
		\node [style=had] (68) at (-9, 10) {};
		\node [] (69) at (-8.5, 9) {};
		\node [] (70) at (-7.5, 9) {};
		\node [] (71) at (-7.5, 9) {};
		\node [] (72) at (-6.5, 9) {};
		\node [] (73) at (-5.5, 9) {};
		\node [] (74) at (-5.5, 9) {};
		\node [] (75) at (-4.5, 9) {};
		\node [] (76) at (-3.5, 9) {};
		\node [] (77) at (-3.5, 9) {};
		\node [] (78) at (-8.5, 2) {};
		\node [] (79) at (-7.5, 2) {};
		\node [] (80) at (-7.5, 2) {};
		\node [] (81) at (-6.5, 2) {};
		\node [] (82) at (-5.5, 2) {};
		\node [] (83) at (-5.5, 2) {};
		\node [] (84) at (-4.5, 2) {};
		\node [] (85) at (-3.5, 2) {};
		\node [] (86) at (-3.5, 2) {};
		\node [] (fl) at (-2.5, 9) {};
		\node [] (fldots) at (-1.5, 9) {$\dots$};
		\node [] (sl) at (-9.5, 2) {};
		\node [] (sldots) at (-10.5, 2) {$\dots$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (4.center) to (32);
		\draw (32) to (28);
		\draw (28) to (33);
		\draw (33) to (31);
		\draw (31) to (29);
		\draw (29) to (30);
		\draw (30) to (6.center);
		\draw (34.center) to (40);
		\draw (40) to (36);
		\draw (39) to (37);
		\draw (37) to (38);
		\draw (38) to (35.center);
		\draw (36) to (39);
		\draw (41.center) to (47);
		\draw (47) to (43);
		\draw (45) to (42.center);
		\draw (46) to (45);
		\draw (46) to (44);
		\draw (44) to (43);
		\draw (48.center) to (54);
		\draw (52) to (49.center);
		\draw (52) to (51);
		\draw (51) to (54);
		\draw (55.center) to (59);
		\draw (58) to (56.center);
		\draw (59) to (58);
		\draw (62) to (61.center);
		\draw (60.center) to (62);
		\draw (63.center) to (64.center);
		\draw (0.center) to (68);
		\draw (68) to (66);
		\draw (66) to (2.center);
		\draw [-stealth] (69.center) to (71.center);
		\draw [-stealth] (72.center) to (74.center);
		\draw [-stealth] (75.center) to (77.center);
		\draw [-stealth] (78.center) to (80.center);
		\draw [-stealth] (81.center) to (83.center);
		\draw [-stealth] (84.center) to (86.center);
		\draw (fl.center) to (fldots);
		\draw [-stealth] (sldots) to (sl.center);
	\end{pgfonlayer}
\end{tikzpicture}


==> Images_eps/tikz_zx_inf.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [] (0) at (0.5, 5.25) {};
		\node [] (1) at (0.5, 6.25) {};
		\node [style=had] (2) at (0.5, 5.75) {};
		\node [] (3) at (2, 4.5) {};
		\node [] (4) at (2, 7) {};
		\node [style=rn] (5) at (2, 5) {$\frac{\pi}{2}$};
		\node [style=rn] (6) at (2, 6.5) {$\frac{\pi}{2}$};
		\node [style=gn] (7) at (2, 5.75) {$\frac{\pi}{2}$};
		\node [] (8) at (1.25, 5.75) {=};
		\node [] (9) at (-1.5, 3.5) {};
		\node [] (10) at (-1, 3.5) {...};
		\node [] (11) at (-0.5, 3.5) {};
		\node [] (12) at (-1.5, 4.5) {};
		\node [] (13) at (-1, 4.5) {...};
		\node [] (14) at (-0.5, 4.5) {};
		\node [style=rn] (15) at (-1, 4) {$\alpha$};
		\node [] (16) at (-0.25, 3.25) {};
		\node [] (17) at (0.25, 3.25) {...};
		\node [] (18) at (0.75, 3.25) {};
		\node [] (19) at (-0.25, 4.25) {};
		\node [] (20) at (0.25, 4.25) {...};
		\node [] (21) at (0.75, 4.25) {};
		\node [style=rn] (22) at (0.25, 3.75) {$\beta$};
		\node [] (23) at (1.75, 3.25) {};
		\node [] (24) at (2.25, 3.25) {...};
		\node [] (25) at (2.75, 3.25) {};
		\node [] (26) at (1.75, 4.25) {};
		\node [] (27) at (2.25, 4.25) {...};
		\node [] (28) at (2.75, 4.25) {};
		\node [style=rn] (29) at (2.25, 3.75) {$\alpha + \beta$};
		\node [] (30) at (1.25, 3.75) {=};
		\node [style=rn] (31) at (4.25, 3.75) {};
		\node [] (32) at (4.25, 3.25) {};
		\node [] (33) at (4.25, 4.25) {};
		\node [] (34) at (4.75, 3.75) {=};
		\node [] (35) at (5.25, 3.25) {};
		\node [] (36) at (5.25, 4.25) {};
		\node [style=gn] (37) at (4.25, 6) {$\alpha$};
		\node [] (38) at (4.25, 5) {};
		\node [] (39) at (4.25, 6.5) {};
		\node [] (40) at (4.75, 5.75) {=};
		\node [style=rn] (41) at (4.25, 5.5) {$\pi$};
		\node [style=gn] (42) at (5.25, 5.5) {$-\alpha$};
		\node [] (43) at (5.25, 6.5) {};
		\node [] (44) at (5.25, 5) {};
		\node [style=rn] (45) at (5.25, 6) {$\pi$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw (0.center) to (2);
		\draw (2) to (1.center);
		\draw (3.center) to (5);
		\draw (5) to (7);
		\draw (7) to (6);
		\draw (6) to (4.center);
		\draw (9.center) to (15);
		\draw (11.center) to (15);
		\draw (15) to (14.center);
		\draw (15) to (12.center);
		\draw (16.center) to (22);
		\draw (18.center) to (22);
		\draw (22) to (21.center);
		\draw (22) to (19.center);
		\draw (15) to (22);
		\draw (23.center) to (29);
		\draw (25.center) to (29);
		\draw (29) to (28.center);
		\draw (29) to (26.center);
		\draw (32.center) to (31);
		\draw (31) to (33.center);
		\draw (36.center) to (35.center);
		\draw (37) to (39.center);
		\draw (38.center) to (41);
		\draw (41) to (37);
		\draw (42) to (44.center);
		\draw (43.center) to (45);
		\draw (45) to (42);
	\end{pgfonlayer}
\end{tikzpicture}


==> Sections/bg_quantum_old.tex <==
Nielsen and Chuang's volume \cite{Nielsen11} is the standard textbook for quantum computing, but this section introduces the core ideas that are needed for the rest of the paper. In quantum mechanics, there are four quantum postulates\footnote{But only three of them are strictly needed: see ``Four Postulates of Quantum Mechanics Are Three'', G. Carcassi {\em et al., Phys. Rev. Lett.} 126, 110402, 2021.} that give us the rules and behaviours that make up quantum systems.

% The quantum postulates
Firstly, a quantum system is represented by a Hilbert space (a complex vector space with inner product) often referred to as a state space. A system's state is described by a unit vector within the Hilbert space. A qubit, the simplest quantum computing system, is represented by 
\begin{align*}
    \ket{\psi} &= \alpha \ket{0} + \beta \ket{1} \\
    &= \alpha \begin{pmatrix} 1 \\ 0 \end{pmatrix} + \beta 
    \begin{pmatrix} 0 \\ 1\end{pmatrix}
\end{align*}
where \Paolo{ $\alpha$ and $\beta$ are complex numbers that satisfy} $|\alpha|^2 + |\beta|^2 = 1$. The dual of a vector is represented by $\bra{\psi} = \ket{\psi}^{T}$.

Secondly, the state space of a composite quantum system is represented by the tensor product of the individual quantum systems. So a system with $n$ quantum systems is represented by ${\ket{\psi_1} \otimes \ket{\psi_2} \otimes \dots \otimes \ket{\psi_n}}$. 
\begin{example}
A 2-qubit system spans a 4-dimensional vector space. This system can represent the Bell state $\frac{1}{\sqrt{2}}(\ket{0}\otimes\ket{0} + \ket{1}\otimes\ket{1}) = \frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$, where the state is represented by the vector $(\frac{1}{\sqrt{2}},0,0,\frac{1}{\sqrt{2}})^T$.
\end{example}


Thirdly, a closed (\ie no interaction with its surrounding environment) quantum system evolves through applications of \textit{unitary operators} on the quantum state $\ket{\psi}$. A unitary operator $U$ is a (linear) transformation such that its inverse is its adjoint $U^{-1} = U^\dagger$. The state after evolution is $U \ket{\psi}$; \Paolo{we recall that unitary operators are norm-preserving transformations}.

Finally, when a quantum system is \textit{measured}, the quantum state randomly \textit{collapses} into one of the states in an orthonormal basis $\{\ket{o_1}, \dots, \ket{o_n}\}$. With the quantum state being $\ket{\psi} = \sum_{i=1}^{n} \alpha_i \ket{o_i}$ and $\sum_{i=1}^{n} |\alpha_i|^2=1$, the probability of the state collapsing to $\ket{o_j}$ is $P(o_j) = |\alpha_j|^2$. After measurement, the quantum state is $\frac{\alpha_j}{|\alpha_j|}{\ket{o_j}}$. It should be noted that measurement can be represented by a set of Hermitian operators $M = \{M_j : 0 \leq j \leq n \}$, where $M_j = \ket{o_j}\bra{o_j}$ is the projector over the one-dimensional space spanned by $\ket{o_j}$.

% Superposition
A quantum state is said to be in \textit{superposition} when it cannot be represented by a single state within an orthonormal basis. I.e. $\ket{\psi}$ is in a superposition in the basis $\{\ket{o_1}, \dots, \ket{o_n}\}$ when $\ket{\psi} \neq \alpha_j \ket{o_j}$ for all $j$.
% Entanglement
Two (or more) quantum systems are \textit{entangled} when the composite quantum state cannot be written as a tensor product of the individual quantum systems.
\begin{example}
The Bell state $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$ cannot be represented by some $\ket{\psi_1} \otimes \ket{\psi_2}$, whereas $\frac{1}{\sqrt{2}}(\ket{00} + \ket{01}) = \ket{0} \otimes \frac{1}{\sqrt{2}} (\ket{0} + \ket{1})$.
\end{example}

% Density Operators and Traces
Whilst representation of a quantum system commonly uses the vector notation given above, it is possible to define the system using a density matrix notation. Given a finite ensemble of quantum systems $\{p_i, \ket{\phi_i}\}$ where the probability of the system being in (pure) state $\ket{\phi_i}$ is $p_i$, the system can be represented by $\rho = \sum_i p_i \ket{\phi_i}\bra{\phi_i}$. This representation changes how the postulates are given. For example, the unitary evolution of the system is given by the so-called {\em super-operator} $U \rho U^\dagger$, where $U$ is a unitary transformation. The trace of a matrix is the sum of the diagonal elements $tr(A) = \sum_i A_{ii}$ and is used in various aspects when working with density matrices (such as measurement).

